Opinion Diffusion and Campaigning on Society Graphs

We study the effects of campaigning, where the society is partitioned into voter clusters and a diffusion process propagates opinions in a network connecting the clusters. Our model is very powerful and can incorporate many campaigning actions, various partitions of the society into clusters, and very general diffusion processes. Perhaps surprisingly, we show that computing the cheapest campaign for rigging a given election can usually be done efficiently, even with arbitrarily-many voters. Moreover, we report on certain computational simulations.

==> junk.tex <==

\item
Perhaps we can show NP-hardness for Plurality (like Proposition~\ref{theorem:borda bsg np hard}); Not clear that we should..
Anyhow, perhaps something like Dominating Set can give it (imagine a dominating set graph, then clone each vertex; then, it shall cost one bribery action to ``flip'' a vertex [like selecting it to be in the dominating set] for it to start eating his neighbors]; and it shall be mandatory to eat the whole graph to win (so probably some other, dummy, non-connected, non-diffusable vertices shall be created on the side)..

\item
We can consider the problem of, given a society graph, determine whether it leads to unique result;
``the same result'' means either (1) the same winner or (2) the same final election.
%
Perhaps (2) is poly-time, by, say, checking whether there are two different vertices that can be eaten in the first day, etc..
Perhaps (1) is NP-hard by something like the Partition reduction. Perhaps not. And perhaps not.

\item
For later I suggest:
\mypara{Force model: subtypes and damping}
One limitation of the model as we have descibed is that it cannot express when voters of one type have different bribery costs.
We could model these two groups by two distinct types, but then we lose the information that they gain confidence from the number of voters of the other type because they share their preferences.
Another limitation is that perhaps the modeling of influence is too crude: every neighboring type exerts the same kind of influence on its neighbors.
However, perhaps voters of type $i$ are strongly influenced by their swap distance $1$ neighbors, but they are also influenced by their swap distance $2$, $3$ etc. neighbors, however with a decreasing power.
A still different issue arises if we try to model socio-economic differences within each type: perhaps the young are influenced differently than the old, but it would not make sense if the influence from old people to young people made them shift their weight, as this would correspond to all the young suddenly becoming old.

To mitigate these problems, we consider the following \emph{force model}.
Let $G$ be a complete directed graph on vertex set $V = [z] \times [\zeta]$, where a vertex $v=(i,j) \in V$ has \emph{type} $i$ and \emph{subtype} $j$.
For each arc $e = (u,v)$ let $p(e) \in [-1, 1]$ be the \emph{power of $u$ over $v$}; if $p(e) > 0$ then $u$ ``pushes'' $v$ and if $p(e) < 0$ it ``pulls'' it.
We say that the \emph{force of $u$ on $v$} is $f(u,v) = w(u) \cdot p((u,v))$.
Intuitively, a vertex $u$ can have large weight $w(u)$ but has small influence over $v$ and thus only applies small force on it.
Then, vertex $u=(i,j)$ shifts its weight to a vertex $v=(i',j')$ with $j = j'$ if $p(v,u) < 0$ and $\sum_{v' = (i',\ell)} f(v', u) > \frac{1}{2} \sum_{v' \in V} f(v', u)$.
The intuition is that $v$ shifts if the total force of a certain type exceeds one half of the total force on $v$, and it always keeps its subtype.

\item
I also suggest this for, say, journal:
Similarly, when approval counts are considered (such as in the \textsc{Support Bribery} problem), a voter type is determined by its preference order and approval count.  

\item
Regarding “totality” of the diffusion: The process can be made more fine-grained by using more types: For example, we can split each original type into three subtypes: “easily influenced”, “hardly influenced”, and “impossible to influence”. Then, perhaps all easily-influenced voters move when more than half of their neighbors have a given preference type; hard to influence voters move if 90$\%$ of their neighbors have a given preference types; and impossible to influence voters never move. We can further say that, once easily-influenced voters change their opinion, they become hard-to-influence voters, and after another move, they become impossible-to-influence (and, of course, one can introduce more levels to this hierarchy). Indeed, our FPT technique works for such a generalized model. Of course, introducing a limit on the number of times a voter changes a point of view gives trivial convergence (but it is also quite natural that at some point people get tired of paying attention to a discussion on a given issue and remain with their fixed preferences). 

\end{itemize}
